SFATTI: Spiking FPGA Accelerator for Temporal Task-driven Inference -- A Case Study on MNIST

Hardware accelerators are essential for achieving low-latency, energy-efficient inference in edge applications like image recognition. Spiking Neural Networks (SNNs) are particularly promising due to their event-driven and temporally sparse nature, making them well-suited for low-power Field Programmable Gate Array (FPGA)-based deployment. This paper explores using the open-source Spiker+ framework to generate optimized SNNs accelerators for handwritten digit recognition on the MNIST dataset. Spiker+ enables high-level specification of network topologies, neuron models, and quantization, automatically generating deployable HDL. We evaluate multiple configurations and analyze trade-offs relevant to edge computing constraints.

==> Config/packages.tex <==
% --- add these two lines *before* the first \usepackage that might touch xcolor ---
\PassOptionsToPackage{table}{xcolor}   % mandate the option
\RequirePackage{xcolor}                % load it exactly once

% now list the rest of your packages in any order, but *remove* the duplicate call
\usepackage{spconf,amsmath,graphicx}
\usepackage[acronym]{glossaries}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{hyperref}
\usepackage{tcolorbox}      % no clash now; xcolor already loaded with table
\usepackage[font=small,skip=10pt]{caption}



\setlength{\textfloatsep}{8pt plus 1.0pt minus 3.0pt}

